Solving weighted and counting variants of connectivity problems parameterized by treewidth deterministically in single exponential time

It is well known that many local graph problems, like Vertex Cover and Dominating Set, can be solved in 2^{O(tw)}|V|^{O(1)} time for graphs G=(V,E) with a given tree decomposition of width tw. However, for nonlocal problems, like the fundamental class of connectivity problems, for a long time we did not know how to do this faster than tw^{O(tw)}|V|^{O(1)}. Recently, Cygan et al. (FOCS 2011) presented Monte Carlo algorithms for a wide range of connectivity problems running in time $c^{tw}|V|^{O(1)} for a small constant c, e.g., for Hamiltonian Cycle and Steiner tree. Naturally, this raises the question whether randomization is necessary to achieve this runtime; furthermore, it is desirable to also solve counting and weighted versions (the latter without incurring a pseudo-polynomial cost in terms of the weights). We present two new approaches rooted in linear algebra, based on matrix rank and determinants, which provide deterministic c^{tw}|V|^{O(1)} time algorithms, also for weighted and counting versions. For example, in this time we can solve the traveling salesman problem or count the number of Hamiltonian cycles. The rank-based ideas provide a rather general approach for speeding up even straightforward dynamic programming formulations by identifying "small" sets of representative partial solutions; we focus on the case of expressing connectivity via sets of partitions, but the essential ideas should have further applications. The determinant-based approach uses the matrix tree theorem for deriving closed formulas for counting versions of connectivity problems; we show how to evaluate those formulas via dynamic programming.

==> deterministic-conclusions.tex <==
\section{Conclusions}
\label{section:conclusions}
In this paper, we have given deterministic algorithms for connectivity problems on graphs of small treewidth, 
with the running time only single exponential in the treewidth. We have given two different techniques.
Each technique solves the standard unweighted versions, but for variants (counting, weighted versions, \ldots), sometimes only one of the techniques appears to be usable.
Both techniques make novel use of classic linear algebra. 
As the treewidth and branchwidth of a graph differ by a constant factor, our algorithms also work
for graphs of bounded branchwidth, and one can easily translate our algorithms to algorithms working on branch decompositions.


Our work improves upon the Cut\&Count approach not only by having deterministic algorithms, but also (some of) our algorithms only use time that is linear in the number of vertices in the graph.
However, the base of the exponent is somewhat larger, and an important question is whether this can be reduced. In the rank-based approach, this amounts to the following question: Can Algorithm~$\mathtt{reduce}$ from the proof of Theorem~\ref{thm:main} be implemented in linear time? It would also be interesting to have a linear time implementation of Algorithm~$\mathtt{reducematchings}$ from Corollary~\ref{thm:mainmatchings}.

We believe that our algorithms not only break a theoretical barrier, but may also be of practical use.
A possible algorithm for e.g., Hamiltonian Circuit may be the following: run the standard DP on the tree decomposition, but as soon as we work with a table of size larger than $2^{\tw}$, 
we can use the rank-based approach and remove table entries by finding a base. Thus, we are
guaranteed that we never have to process  tables of size larger than $2^{\tw}$, at the cost
of running a number of Gaussian elimination steps. 
It would be very interesting to perform an algorithm engineering study on this approach.
It also may be interesting to see how this combines with a well known heuristic by Cook and Seymour for TSP~\cite{DBLP:journals/informs/CookS03}, that uses finding a minimum length Hamiltonian Circuit in a graph with small branchwidth as a central step.
%William Cook, Paul D. Seymour: Tour Merging via Branch-Decomposition. INFORMS Journal on Computing 15(3): 233-248 (2003)

A final very intriguing question that our work implies is the following: Is the rank-based approach also 
usable in settings outside graphs of small treewidth? The rank-based approach gives a new twist to the dynamic programming approach, in the sense that we consider the ``algebraic structure'' of the partial certificates in a quite novel way. Thus, this suggests a study of this algebraic structure for dynamic programming algorithms for problems in other areas.

We would like to mention that uses of the rank based approach could also be found in work on rank-width boolean-width~\cite{Oum2006514,DBLP:journals/tcs/Bui-XuanTV11}, but in these cases the rank structure exploited is by more explicit assumption present in the input.

\section*{Acknowledgements}

We would like to thank Piotr Sankowski for pointing us to relevant literature of matrix-multiplication time algorithms.
Moreover the second author thanks Marcin Pilipczuk and \L{}ukasz Kowalik for helpful discussions at the early stage of the paper.


==> packages.tex <==

\usepackage[utf8x]{inputenc}

\usepackage{tikz}
\usepackage{rotating}
\usepackage{xspace}
\usepackage{array}
\usepackage{paralist}
\usepackage{fullpage}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{etex}
\usepackage{graphicx}
\usepackage{paralist}

\usepackage[noend]{algorithmic}
\usepackage[boxed]{algorithm}

\usepackage{color}

\usepackage{fullpage}
